Knowledge-augmented Pre-trained Language Models for Biomedical Relation Extraction

Automatic relationship extraction (RE) from biomedical literature is critical for managing the vast amount of scientific knowledge produced each year. In recent years, utilizing pre-trained language models (PLMs) has become the prevalent approach in RE. Several studies report improved performance when incorporating additional context information while fine-tuning PLMs for RE. However, variations in the PLMs applied, the databases used for augmentation, hyper-parameter optimization, and evaluation methods complicate direct comparisons between studies and raise questions about the generalizability of these findings. Our study addresses this research gap by evaluating PLMs enhanced with contextual information on five datasets spanning four relation scenarios within a consistent evaluation framework. We evaluate three baseline PLMs and first conduct extensive hyperparameter optimization. After selecting the top-performing model, we enhance it with additional data, including textual entity descriptions, relational information from knowledge graphs, and molecular structure encodings. Our findings illustrate the importance of i) the choice of the underlying language model and ii) a comprehensive hyperparameter optimization for achieving strong extraction performance. Although inclusion of context information yield only minor overall improvements, an ablation study reveals substantial benefits for smaller PLMs when such external data was included during fine-tuning.

==> figures/model_baseline.tex <==
\begin{figure}[tb]
\includesvg[]{figures/model_baseline.svg}
\centering
\caption{%
Illustration of the baseline model using the example of chemical-protein relation extraction. 
%
We build one input example per entity pair, i.e., chemical-protein pair, in each sentence and mark the pair under investigation with special tokens (i.e., [HEAD-S],[HEAD-E],[TAIL-S] and [TAIL-E]).
%
The sentence is embedded with a pretrained language model. 
%
Finally, the embedding of the [CLS] special token is passed through an output layer performing the relation classification.
}
\label{5:fig:model_baseline}
\end{figure}

==> figures/model_kge.tex <==
\begin{figure}[tbhp]
\includesvg[]{figures/model_kge.svg}
\centering
\caption{%
Illustration of the model augmented with additional embedded entity information.
%
First, we lookup the pre-trained knowledge base embeddings for the head and tail entity under investigation and input the concatenation of both to a multi-layer perceptron (MLP).
%
The resulting embedding is concatenated to the contextualized input text embedding as additional input to the classification layer.
%
}
\label{5:fig:model_kge}
\end{figure}

==> figures/model_str.tex <==
\begin{figure}[tbhp]
\includesvg[]{figures/model_str.svg}
\centering
\caption{%
Illustration of the model extended with molecular  information of chemicals.
%
For a given chemical $c$, we first retrieve it's respective SMILES string $SM_c$, prepend the [CLS] token to $SM_c$ and feed it into the compound language model.
%
We use the representation of the [CLS] token in the last hidden layer as encoding for the structure of $c$.
%
Finally, we concatenate the structure embedding with the language model's output to form the classification layer's input.
}
\label{5:fig:model_str}
\end{figure}

==> figures/model_text.tex <==
\begin{figure}[tbhp]
\includesvg[]{figures/model_text.svg}
\centering
\caption{%
Illustration of the model augmented with additional textual entity information. 
%
We conduct knowledge base lookups (in this case CTD chemicals) to retrieve textual descriptions for the head entity, the tail entity or both using entity identifiers (here MESH identifiers).
%
When working with data sets that include entity normalizations, we employ them; otherwise, we resort to exact string matching to locate the entity identifier associated with a specific mention.
%
We include the textual descriptions by appending them to the input text separated by then [SEP] token.
}
\label{5:fig:model_text}
\end{figure}
